Escape of photons from two fixed extreme Reissner-Nordstr\"om black holes

We study the scattering of light (null geodesics) by two fixed extreme Reissner-Nordstr\"om black holes, in which the gravitational attraction of their masses is exactly balanced with the electrostatic repulsion of their charges, allowing a static spacetime. We identify the set of unstable periodic orbits that constitute the fractal repeller that completely describes the chaotic escape dynamics of photons. In the framework of periodic orbit theory, the analysis of the linear stability of the unstable periodic orbits is used to obtain the main quantities of chaos that characterize the escape dynamics of the photons scattered by the black holes. In particular, the escape rate which is compared with the result obtained from numerical simulations that consider statistical ensembles of photons. We also analyze the dynamics of photons in the proximity of a perturbed black hole and give an analytical estimation for the escape rate in this system.

==> response_3.tex <==
Dear Editor,

Thank you for your message enclosing the referee's report on our
manuscript

Re: DA10275, 
    ``Escape of photons from two fixed extreme Reissner-Nordstr\"{o}m
    black holes''
    by Daniel Alonso, Antonia Ruiz, and Manuel S\'anchez-Hern\'andez.

We thank the referee for her/his review and clarifying points.

Please find below our reply to the referee's comments. The list of changes is 
also provided.

Reply to the referee's comments:

i.- In respond to the point (i), the increase with the separation d of the
escape rate evaluated in the killing time is a transient behavior before the
global decrease at large d. To show that, in Figure (9) we have extended our 
numerical computations of the escape rate to larger distances d, both in the 
killing time and the affine parameter. In both cases the escape rate decreases 
asymptotically with d. This behavior has also been observed in other scattering 
systems, such as the four hard disk scatterers. In general the escape rate at 
large distance d decrease as f(d)/d, being f(d) a function determined by the
scattering interaction potential and 1/d is the contribution of the time of 
flight. Please note that the escape rate is given per unit time.

This explanation has been inserted in a new brief paragraph at the end of 
Section VI, where the new Figure (9) is referred, and appropiate references are
also given.

ii.- In respond to the point (ii), concerning the escape rate values represented 
in Figures 8 and 9, we have improved our numerical computations by increasing the 
number of particles that we integrate in the simulations.

List of changes:

1.- The Figure 9 has been modified, new values of the escape rate for larger
separation distance d has been included.

2.- A brief new paragraph refering to the new points in Figure 9 has been 
inserted at the end of Section VI.

Yours sincerely,

